A Dynamic Fusion Model for Consistent Crisis Response

In response to the urgent need for effective communication with crisis-affected populations, automated responses driven by language models have been proposed to assist in crisis communications. A critical yet often overlooked factor is the consistency of response style, which could affect the trust of affected individuals in responders. Despite its importance, few studies have explored methods for maintaining stylistic consistency across generated responses. To address this gap, we propose a novel metric for evaluating style consistency and introduce a fusion-based generation approach grounded in this metric. Our method employs a two-stage process: it first assesses the style of candidate responses and then optimizes and integrates them at the instance level through a fusion process. This enables the generation of high-quality responses while significantly reducing stylistic variation between instances. Experimental results across multiple datasets demonstrate that our approach consistently outperforms baselines in both response quality and stylistic uniformity.

==> latex/Table/Main_performance.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lllccccc}
% \toprule
% \textbf{Model} & \textbf{Category} & \textbf{Method} & \textbf{Professionalism} & \textbf{Actionability} & \textbf{Relevance} & \textbf{Consistency} & \textbf{Overall Quality} \\
% \midrule

% \multirow{8}{*}{Llama}
% & \multirow{3}{*}{Baseline} & IP & 0.74 (0.33) & 0.52 (0.36) & 0.80 (0.02) & 0.24 & 0.66 \\
% &                            & RAG & 0.96 (0.14) & 0.63 (0.33) & 0.80 (0.02) & 0.16 & 0.80 \\
% &                            & RAG-PE & 0.94 (0.19) & 0.50 (0.14) & 0.80 (0.02) & 0.12 & 0.74 \\
% \cdashline{3-8}

% & \multirow{5}{*}{Fusion}    & Prompt and Select & 0.50 (0.50) & 0.98 (0.14) & 0.79 (0.02) & 0.22 & 0.75 \\
% &                            & Fusion wo Eval & 0.55 (0.27) & 0.97 (0.16) & 0.79 (0.02) & 0.15 & 0.77 \\
% &                            & Fusion w Eval & 0.98 (0.10) & 0.77 (0.27) & 0.79 (0.02) & 0.13 & 0.86 \\
% &                            & Fusion w Eval \& Instruct & 0.92 (0.19) & 0.99 (0.07) & 0.79 (0.02) & 0.09 & 0.92 \\
% &                           \rowcolor{gray!20} & Fusion w Eval \& Weight Instruct & 0.99 (0.07) & 0.99 (0.09) & 0.79 (0.02) & \textbf{\underline{0.06}} & \textbf{\underline{0.95}} \\

% \midrule
% \multirow{8}{*}{Misnistral}
% & \multirow{3}{*}{Baseline} & IP & 0.87 (0.34) & 0.98 (0.15) & 0.79 (0.02) & 0.17 & 0.90 \\
% &                            & RAG & 0.87 (0.22) & 0.97 (0.11) & 0.81 (0.03) & 0.12 & 0.90 \\
% &                            & RAG-PE & 0.76 (0.26) & 0.96 (0.15) & 0.80 (0.02) & 0.14 & 0.85 \\
% \cdashline{3-8}

% & \multirow{5}{*}{Fusion}    & Prompt and Select & 0.75 (0.39) & 0.81 (0.39) & 0.80 (0.03) & 0.27 & 0.78 \\
% &                            & Fusion wo Eval & 0.93 (0.25) & 1.00 (0.04) & 0.80 (0.02) & 0.10 & 0.93 \\
% &                            & Fusion w Eval & 0.92 (0.28) & 1.00 (0.08) & 0.80 (0.02) & 0.13 & 0.93 \\
% &                            & Fusion w Eval \& Instruct & 0.96 (0.13) & 1.00 (0.05) & 0.80 (0.02) & 0.07 & 0.94 \\
% &                           \rowcolor{gray!20} & Fusion w Eval \& Weight Instruct & 0.97 (0.13) & 1.00 (0.08) & 0.80 (0.02) & 0.08 & 0.95 \\

% \midrule
% \multirow{8}{*}{Qwen}
% & \multirow{3}{*}{Baseline} & IP & 0.98 (0.13) & 0.99 (0.06) & 0.81 (0.02) & 0.07 & 0.95 \\
% &                            & RAG & 0.79 (0.28) & 0.86 (0.31) & 0.81 (0.03) & 0.21 & 0.82 \\
% &                            & RAG-PE & 0.63 (0.31) & 0.86 (0.31) & 0.80 (0.03) & 0.22 & 0.76 \\
% \cdashline{3-8}
% & \multirow{5}{*}{Fusion}    & Prompt and Select & 0.85 (0.36) & 0.99 (0.10) & 0.81 (0.02) & 0.16 & 0.90 \\
% &                            & Fusion wo Eval & 0.90 (0.30) & 0.99 (0.11) & 0.81 (0.02) & 0.14 & 0.92 \\
% &                            & Fusion w Eval & 0.99 (0.06) & 1.00 (0.12) & 0.81 (0.02) & 0.07 & 0.96 \\
% &                            & Fusion w Eval \& Instruct & 0.98 (0.15) & 0.99 (0.10) & 0.81 (0.02) & 0.09 & 0.95 \\
% &                            & Fusion w Eval \& Weight Instruct & 0.98 (0.15) & 1.00 (0.09) & 0.81 (0.02) & 0.09 & 0.95 \\

% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison (mean and standard deviation) of different methods across models}
% \label{tab:model_grouped_mean_std_with_category}
% \end{table*}
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lllccccc}
\toprule
\textbf{Model} & \textbf{Category} & \textbf{Method} & \textbf{Professionalism} & \textbf{Actionability} & \textbf{Relevance} & \textbf{Consistency} & \textbf{Overall Quality} \\
\midrule

\multirow{8}{*}{Llama}
& \multirow{5}{*}{Baseline} & Instructional Prompt  & 0.74 (0.33) & 0.52 (0.36) & 0.80 (0.02) & 0.24 & 0.66 \\
&                            & RAG & 0.96 (0.14) & 0.63 (0.33) & 0.80 (0.02) & 0.16 & 0.80 \\
&                            & RAG-PE & 0.94 (0.19) & 0.50 (0.14) & 0.80 (0.02) & 0.12 & 0.74 \\

&                            & Prompt and Select & 0.50 (0.50) & 0.98 (0.14) & 0.79 (0.02) & 0.22 & 0.75 \\
&                            & Fusion wo Eval & 0.55 (0.27) & 0.97 (0.16) & 0.79 (0.02) & 0.15 & 0.77 \\
\cdashline{3-8}
&  \multirow{3}{*}{Fusion}   & Fusion w Eval & 0.98 (0.10) & 0.77 (0.27) & 0.79 (0.02) & 0.13 & 0.86 \\
&                            & Fusion w Eval \& Instruct & 0.92 (0.19) & 0.99 (0.07) & 0.79 (0.02) & 0.09 & 0.92 \\
% \rowcolor{gray!15}
&                            & \cellcolor{gray!15}Fusion w Eval \& Weight Instruct & \cellcolor{gray!15}\textbf{0.99 (0.07)} & \cellcolor{gray!15}\textbf{0.99 (0.09)} & \cellcolor{gray!15}\textbf{0.79 (0.02)} & \cellcolor{gray!15}\textbf{0.06} & \cellcolor{gray!15}\textbf{0.95} \\

\midrule
\multirow{8}{*}{Mistral}
& \multirow{5}{*}{Baseline} & Instructional Prompt  & 0.87 (0.34) & 0.98 (0.15) & 0.79 (0.02) & 0.17 & 0.90 \\
&                            & RAG & 0.87 (0.22) & 0.97 (0.11) & 0.81 (0.03) & 0.12 & 0.90 \\
&                            & RAG-PE & 0.76 (0.26) & 0.96 (0.15) & 0.80 (0.02) & 0.14 & 0.85 \\

&                            & Prompt and Select & 0.75 (0.39) & 0.81 (0.39) & 0.80 (0.03) & 0.27 & 0.78 \\
&                            & Fusion wo Eval & 0.93 (0.25) & 1.00 (0.04) & 0.80 (0.02) & 0.10 & 0.93 \\
\cdashline{3-8}
&  \multirow{3}{*}{Fusion}                           & Fusion w Eval & 0.92 (0.28) & 1.00 (0.08) & 0.80 (0.02) & 0.13 & 0.93 \\
&                            & Fusion w Eval \& Instruct & 0.96 (0.13) & 1.00 (0.05) & 0.80 (0.02) & \textbf{0.07} & 0.94 \\
% \rowcolor{gray!15}
&                            & \cellcolor{gray!15}Fusion w Eval \& Weight Instruct & \cellcolor{gray!15}\textbf{0.97 (0.13)} & \cellcolor{gray!15}\textbf{1.00 (0.08)} & \cellcolor{gray!15}\textbf{0.80 (0.02)} & \cellcolor{gray!15}0.08 & \cellcolor{gray!15}\textbf{0.95} \\


\bottomrule
\end{tabular}
}
\caption{Performance comparison (mean and standard deviation) of different methods across models. For consistency, a lower value means better consistency.
Best results per model are highlighted in gray.}
\label{main_performance}
\end{table*}


==> latex/Table/Tem.tex <==
\begin{table}[h]
\resizebox{0.48\textwidth}{!}{
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Setup} & \textbf{Pro} & \textbf{Act} & \textbf{Rel} & \textbf{Consist} \\
\midrule
\textsc{Temperature 0.4} & 0.41 & 0.40 & 0.02 & \textbf{0.28} \\
\textsc{Temperature 0.5} & 0.48 & 0.24 & 0.02 & \textbf{0.25} \\
\textsc{Temperature 0.6} & 0.33 & 0.36 & 0.02 & \textbf{\underline{0.24}} \\
\textsc{Temperature 0.7} & 0.30 & 0.39 & 0.02 & \textbf{\underline{0.24}} \\
\textsc{Temperature 0.8} & 0.38 & 0.43 & 0.02 & \textbf{0.28} \\
\bottomrule
\end{tabular}}
\caption{Consistency across different decoding temperatures.}
\label{tab:temperature-results}
\end{table}


==> latex/Table/generalization.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{Professionalism} & \textbf{Actionability} & \textbf{Relevance} & \textbf{Consistency} & \textbf{Overall Quality} \\
\midrule
\rowcolor{blue!5}
\multicolumn{6}{c}{\textbf{Baseline Methods}} \\
\addlinespace

Instructional Prompt  & 0.93 (0.24) & 0.94 (0.23) & 0.79 (0.02) & 0.16 & 0.91 \\
RAG & 0.94 (0.23) & 0.97 (0.12) & 0.77 (0.02) & 0.12 & 0.92 \\
RAG-PE & 0.76 (0.39) & 0.72 (0.40) & 0.77 (0.02) & 0.27 & 0.75 \\

Prompt and Select & 0.97 (0.12) & 0.98 (0.12) & 0.77 (0.02) & 0.09 & 0.93 \\
Fusion wo Eval & 0.96 (0.21) & 0.97 (0.13) & 0.78 (0.02) & 0.12 & 0.93 \\
% \midrule
% \cdashline{1-6}
\rowcolor{blue!5}
\multicolumn{6}{c}{\textbf{Fusion-Based Methods}} \\
Fusion w Eval & 0.98 (0.10) & 0.98 (0.11) & 0.78 (0.02) & 0.08 & 0.94 \\
Fusion w Eval \& Instruct & 0.96 (0.15) & 0.97 (0.15) & 0.78 (0.02) & 0.11 & 0.93 \\
Fusion w Eval \& Weight Instruct & \textbf{1.00 (0.00)} & \textbf{0.99 (0.11)} & 0.78 (0.02) & \textbf{0.04} & \textbf{0.95} \\
\bottomrule
\end{tabular}
}
\caption{Cross-crisis generalization performance, which includes response to earthquake and typhoon. }
\label{table:Generalization}
\end{table*}

==> latex/Table/human_eval_reliability.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Metric} & \textbf{Instructional Prompt} & \textbf{RAG} & \textbf{Fusion w/ Eval \& Weight Instruct} \\
\midrule
Agreement Rate & 0.86 & 0.72 & 0.78 \\
Cohen’s Kappa  & 0.76 & 0.60 & 0.62 \\
\bottomrule
\end{tabular}}
\caption{Inter-annotator agreement (Agreement Rate and Cohen’s Kappa) across three strategies.}
\label{tab:agreement}
\end{table}

